On Irradiance Distributions for Weakly Turbulent FSO Links: Log-Normal vs. Gamma-Gamma

Weak turbulence is commonly modeled using the log-normal distribution. Our experimental results show that this distribution fails to capture irradiance fluctuations in this regime. The Gamma-Gamma model is shown to be more accurate.

==> Sections/AreaNueva.tex <==
\usetikzlibrary {arrows.meta}

\begin{tikzpicture} [scale=1]

\definecolor{my_blue}{rgb}{0.87,0.92,0.98}
\definecolor{my_b}{rgb}{0.67,0.75,0.98}
\definecolor{my_b2}{rgb}{0.53,0.64,0.93}
\definecolor{my_g}{rgb}{0.09,0.71,0.14}

\begin{axis}[
%every axis/.append style = {font=\footnotesize},
%width=4in,  %ancho de la figura
width=1\textwidth,
    height=3.2in,   %alto de la figura
% ymode = log,
xmin = 0.12,
xmax = 0.35,
ymin = 0.03,
ymax = 1.4,
xlabel = {$\sigma_s$~[m]},
ylabel = {$\sigma_R^2$},
ylabel shift=-2ex,
xlabel shift=-2ex,
grid = major,
grid style = {dashed,lightgray!75},
ytick = {0.2,0.4,...,1.2},
xtick={0.12,0.15,0.2,0.25,0.3,0.35},
]

\addplot [name path=lim, color=black, very thick]
   coordinates {
         (0,1) (1.2,1)};


\addplot [name path=R2,color=my_b2,solid,line width=0.75pt,mark options={solid}]
   coordinates {
         (0.12,0)(0.35,0)};

\addplot [name path=R2_Error,color=red,solid,line width=0.75pt,mark options={solid}]
   coordinates {
         (0,0)(0.117,0.01)(0.12,0.05) (0.13,0.1 )(0.148,0.2)(0.16,0.3)(0.17,0.4 )(0.18,0.5)(0.187,0.6)(0.194,0.7) (0.2,0.8) (0.205,0.9) (0.21,1)};
        
%----------------------------------------
\addplot[my_b2, opacity=0.3] fill between[of=R2 and lim];

\addplot[red, opacity=0.3] fill between[of=R2_Error and lim];


%\addplot [only marks,thin, color=black, mark=x, mark options={solid, scale=1.8}]coordinates {(0.35,0.8)};

\addplot [only marks,thin, color=blue, mark=*, mark options={solid, scale=1}]  coordinates { (0.25,1)};
\addplot [only marks,thin, color=orange, mark=*, mark options={solid, scale=1}]  coordinates { (0.25,0.5)};
\addplot [only marks,thin, color=blue, mark=*, mark options={solid, scale=1.5}]  coordinates { (0.25,0.1)};
        
\addplot [only marks, color=my_g, mark=* , mark options={solid, scale=1}]
   coordinates {
        (0.12,1)};    
\addplot [only marks, color=blue, mark=* , mark options={solid, scale=1}]
   coordinates {
        (0.12,0.5)};  
\addplot [only marks, color=blue, mark=* , mark options={solid, scale=1}]
   coordinates {
        (0.12,0.1)};  

\addplot [only marks, color=blue, mark=* , mark options={solid, scale=1.5}]
   coordinates {
        (0.35,1)};  
\addplot [only marks, color=blue, mark=* , mark options={solid, scale=1.5}]
   coordinates {
        (0.35,0.5)};  
\addplot [only marks, color=magenta, mark=* , mark options={solid, scale=2.2}]
   coordinates {
        (0.35,0.1)};  
                
%\addplot [only marks,thin, color=black, mark=x, mark options={solid, scale=1.8}]coordinates {(0.15,0.1)};    


\end{axis}


\node at (1.4,0.12)(input) {};

\node at ($(input.south)+(0.9,16em)$)[font=\scriptsize] {Numerical instability};
\node at ($(input.south)+(0.8,15.2em)$)[font=\scriptsize]  {of PDF to compute BER};
\draw[->] ($(input.south)+(0.8,14.8em)$)-- ($(input.south)+(0.4,11em)$);


\node at (3.7,1.6) [font=\scriptsize]{ Impact pointing errors};
\node at ($(input.south)+(0.8,3.7em)$) [font=\scriptsize]{ -};
\node at ($(input.south)+(3.9,3.7em)$)  [font=\scriptsize]{ +};
\draw[->,font=\scriptsize]  ($(input.south)+(1,3.7em)$) --  ($(input.south)+(3.7,3.7em)$);

\node [draw,fill=white,anchor= south west,font=\scriptsize] at ($(input.south)+(0.2,17em)$){\shortstack[l]{ 
Strong Turbulence ($\sigma_R^2>1$)}};

%BERs
\node at ($(input.south)+(4.3,14em)$)[font=\scriptsize] {$\Delta\approx0.02$~dB };
\node at ($(input.south)+(4.25,7.3em)$) [font=\scriptsize] {$\Delta\approx0.035$~dB };
\node at ($(input.south)+(4.3,1.8em)$) [font=\scriptsize] {$\Delta\approx0.17$~dB };
\node at ($(input.south)+(2.3,14em)$)[font=\scriptsize]  {$\Delta\approx0.004$~dB };
\node at ($(input.south)+(2.3,7.3em)$) [font=\scriptsize] {$\Delta\approx0.006$~dB };
\node at ($(input.south)+(2.3,1.8em)$) [font=\scriptsize]  {$\Delta\approx0.024$~dB };
\node at ($(input.south)+(-0.8,14em)$) [font=\scriptsize] {$\Delta\approx0$~dB };
\node at  ($(input.south)+(-0.8,7.3em)$)[font=\scriptsize]  {$\Delta\approx0$~dB };
\node at  ($(input.south)+(-0.8,1.8em)$) [font=\scriptsize] {$\Delta\approx0$~dB };


\end{tikzpicture}%

==> Sections/FigBER.tex <==
    \begin{tikzpicture}[scale=1]    

\definecolor{my_pink}{rgb}{1,0.07,0.65}
\definecolor{my_g}{rgb}{0.09,0.71,0.14}
\definecolor{FEC}{rgb}{0.5, 0.0, 0.13}

\definecolor{fuchsia}{rgb}{0.6,0.4,0.8}

\begin{semilogyaxis}[ 
    width=0.6\textwidth,
    height=3.3in,   %alto de la figura
    xmin=-4, xmax=16,
    ymin=1e-5, ymax=3e-1,  %similar a eje X
    xlabel={Transmitted Power $P$~[dBm]}, %Nombre eje X
    ylabel shift=-4ex,
    xlabel shift=-4ex,
    font=\small,
    ylabel={Average BER~$\bar{P_\text{b}}$}, %Nombre eje X
    xtick={-4,-2,...,16},    %Similar al ajuste del grid del eje X, pero cuidado, porque es logarítmico 
    grid=major,
    grid style={dashed,lightgray!75},
]

%----------LEYENDA-----------------
\addplot [color=black,solid,line width=1pt,mark options={solid}]coordinates {
         (10,1) (10,2)};\label{Orig_var1_jit12_black}
\addplot [color=black,dashed,line width=1pt,mark options={solid}]coordinates {
         (10,1) (10,2)};\label{Dashed_black}
\addplot [color=black,dotted,line width=1pt,mark options={solid}]coordinates {(10,1) (10,2)};\label{dotted_black}
 \addplot [only marks, color=black, mark=*, mark options={solid,scale=0.8, fill=white}]coordinates {(0.35,1)};\label{MC}
\addplot [name path=lim, color=FEC, very thick]
coordinates {(10,1) (10,2)}; \label{FEClimit}


%------------FEC LIMIT
  \addplot [name path=lim, color=FEC, very thick]
   coordinates {(-10,3.84e-3) (16,3.84e-3)};
  
%-------varR=0.9 Jiiter=0.2-------------

\addplot [color=my_g,solid,line width=1pt,mark options={solid}]file{./txtData/BER_3km/BER_orig_varR09_jit2.txt};

\addplot [ color=my_g,dashed,line width=1pt,mark options={solid}] file {./txtData/ICTON/Aprox2_varR09_jit2.txt};

\addplot [color=my_g,dotted,line width=1pt,mark options={solid}] file{./txtData/UpperBound/Aprox2_varR09_jit2.txt};

%----MONTE CARLO----
\addplot [only marks, color=my_g, mark=*, mark options={solid,scale=0.8, fill=white}]file{./txtData/MC_3km/BER_MC_varR09_jit2.txt};\


%-----varR=0.1---jitter 0.35-----

\addplot [color=my_pink,solid,line width=1pt,mark options={solid}]file{./txtData/BER_3km/BER_orig_varR01_jit35.txt};\label{Orig_var01_jit35}

\addplot [ color=my_pink,dotted,line width=1pt,mark options={solid}] file{./txtData/UpperBound/varR01_jit35/OOK_aprox2.txt};
    
\addplot [color=my_pink,dashed,line width=1pt,mark options={solid}] file{./txtData/ICTON/Aprox2_varR01_jit35_new.txt};


%----MONTE CARLO----

\addplot [only marks, color=my_pink, mark=*, mark options={solid,fill=white,scale=0.8}]file{./txtData/MC_3km/BER_MC_orig_varR01_jit35.txt};\label{MC_orig_var01_jit35}



%------varR0.5------JITTER 0.25--------------

\addplot [color=orange,solid,line width=1pt,mark options={solid}] file {./txtData/BER_3km/BER_orig_varR05_jit25.txt};\label{Orig_var05_jit25}

\addplot [color=orange,dotted,line width=1pt,mark options={solid}] file{./txtData/UpperBound/varR05_jit25/OOK_aprox2.txt};
    
\addplot [color=orange,dashed,line width=1pt,mark options={solid}] file{./txtData/ICTON/Aprox2_varR05_jit25.txt};


%----MONTE CARLO----
\addplot [only marks, color=orange, mark=*, mark options={solid,scale=0.8,fill=white}]file{./txtData/MC_3km/BER_MC_orig_varR05_jit25.txt};\label{MC_orig_var05_jit25}

 
\end{semilogyaxis} %Finalizamos el diseño de la gráfica en sí


\node [draw,fill=white,anchor= south west,font=\scriptsize] at (5.1,5.1) {\shortstack[l]{ 
\ref{Orig_var1_jit12_black} \hspace{0.01cm} \eqref{eq:BER_LN}: Exact \\
 \ref{dotted_black} \hspace{0.01cm}  \eqref{eq:BER_Approx2_UpperBound}: \textbf{This work}\\
\ref{Dashed_black} \hspace{0.01cm}  \eqref{eq:BER_Aprox2_ICTON}: \cite{ICTON}\\
\hspace{0.17cm}   \ref{MC} \hspace{0.3cm}  Monte Carlo\\
  \ref{FEClimit} \hspace{0.01cm}  HD-FEC limit}};


\node [coordinate](input) {};

%DELTA
\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(2.03,11.1em)$) -- ($(input.north)+(2.03,13em)$);
\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(2.42,11.1em)$) -- ($(input.north)+(2.42,13em)$);
 \node at ($(input.north) + (2.15, 13.5 em)$) [ scale=1, font=\scriptsize] {$0.94$~dB};

\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(4.5,11.1em)$) -- ($(input.north)+(4.5,13em)$);
\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(4.76,11.1em)$) -- ($(input.north)+(4.76,13em)$);
 \node at ($(input.north) + (4.6, 13.5em)$) [ scale=1, font=\scriptsize] {$0.7$~dB};


\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(3.4,11.1em)$) -- ($(input.north)+(3.4,13em)$);
\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(3.58,11.1em)$) -- ($(input.north)+(3.58,13em)$);
 \node at ($(input.north) + (3.25, 13.5 em)$) [scale=1, font=\scriptsize] {$0.4$ dB};

%DELTA2
\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(2.03,11.1em)$) -- ($(input.north)+(2.03,9.3em)$);
\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(2.11,11.1em)$) -- ($(input.north)+(2.11,9.3em)$);
\node at ($(input.north) + (1.6, 8.9 em)$) [ scale=1, font=\scriptsize] {$\Delta\approx0.21$~dB};

\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(4.5,11.1em)$) -- ($(input.north)+(4.5,9.3em)$);
\node at ($(input.north) + (4.8, 8.9em)$) [scale=1, font=\scriptsize] {$\Delta\approx0.08$~dB};

\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(3.4,9.3em)$) -- ($(input.north)+(3.4,11.2em)$);
\node at ($(input.north) + (3.3, 8.9 em)$) [scale=1, font=\scriptsize] {$\Delta\approx0.1$ dB};


%\draw[latex-,solid, black,line width=0.5pt] ($(input.north)+(6.1,8.5em)$) -- ($(input.north)+(2.5,6em)$);
\draw[stealth-,solid, black,line width=1pt,rounded corners]($(input.north)+(3.5,16em)$) -- ($(input.north)+(1.1,14.5em)$);
\node at ($(input.north) + (4.2, 16.7 em)$) [scale=1.2, font=\scriptsize] {Increasing};
\node at ($(input.north) + (4.2, 16 em)$) [scale=1.2, font=\scriptsize] {Turbulence};


\node at ($(input.north) + (1.75, 5.9em)$) [scale=1.2, font=\scriptsize] {High pointing};
\node at ($(input.north) + (1.9, 5.1em)$) [scale=1.2, font=\scriptsize] {errors};
\node at ($(input.north) + (7.15, 5.9em)$) [scale=1.2, font=\scriptsize] {Low pointing};
\node at ($(input.north) + (7.2, 5.1em)$) [scale=1.2, font=\scriptsize] {errors};
\draw[stealth-,solid, black,line width=1pt,rounded corners] ($(input.north)+(6.7,5.4em)$) -- ($(input.north)+(2.6,5.4em)$);
%DELTA2
% \draw[-,dashed, black,line width=0.5pt] ($(input.north)+(2.22,9.4em)$) -- ($(input.north)+(2.22,10.7em)$);
% \draw[-,dashed, black,line width=0.5pt] ($(input.north)+(2.29,9.4em)$) -- ($(input.north)+(2.29,10.7em)$);
% \node at ($(input.north) + (2.28, 11 em)$) [color=red, scale=1, font=\scriptsize] {$\Delta_2\approx0.21$ dB};

% \draw[-,dashed, black,line width=0.5pt] ($(input.north)+(4.6,9.3em)$) -- ($(input.north)+(4.6,11.9em)$);
% \node at ($(input.north) + (4.8, 12.4 em)$) [color=red, scale=1, font=\scriptsize] {$\Delta_2\approx0.1$ dB};

% \draw[-,dashed, black,line width=0.5pt] ($(input.north)+(3.35,9.3em)$) -- ($(input.north)+(3.35,11.7em)$);
% \node at ($(input.north) + (3.4, 11.8 em)$) [color=red, scale=1, font=\scriptsize] {$\Delta_2\approx0.08$ dB};

%Ellipse
\node[ellipse,line width=0.75pt, draw,minimum width = 0.6cm, 
	minimum height = 0.05cm, rotate=45] (e) at (3.25,1) {};
\node at ($(input.north) + (2.4, 2em)$) [scale=1, font=\scriptsize] {$\sigma_s=0.35$ m};
\node at ($(input.north) + (2.5, 1.3em)$) [scale=1, font=\scriptsize] {$\sigma_R^2=0.1$};
 
\node[ellipse,line width=0.75pt, draw,minimum width = 0.6cm, 
	minimum height = 0.05cm,rotate=45] (e) at (7.1,1) {};
\node at ($(input.north) + (6.3, 2em)$) [scale=1, font=\scriptsize] {$\sigma_s=0.2$ m};
\node at ($(input.north) + (6.3, 1.3em)$) [scale=1, font=\scriptsize] {$\sigma_R^2=0.9$};

\node[ellipse,line width=0.75pt, draw,minimum width = 0.6cm, 
	minimum height = 0.05cm,rotate=45] (e) at (5.4,1) {};
\node at ($(input.north) + (4.6,1.7em)$) [scale=1, font=\scriptsize] {$\sigma_s=0.25$ m};
\node at ($(input.north) + (4.6, 1em)$) [scale=1, font=\scriptsize] {$\sigma_R^2=0.5$};
 
\end{tikzpicture}

==> Sections/FigBER_newPDF.tex <==
    \begin{tikzpicture}[scale=1]    

\definecolor{my_pink}{rgb}{1,0.07,0.65}
\definecolor{my_g}{rgb}{0.09,0.71,0.14}
\definecolor{FEC}{rgb}{0.5, 0.0, 0.13}

\definecolor{fuchsia}{rgb}{0.6,0.4,0.8}

\begin{semilogyaxis}[ 
    width=1\textwidth,
    height=3.2in,   %alto de la figura
    xmin=-5, xmax=13,
    ymin=5e-5, ymax=3e-1,  %similar a eje X
    xlabel={Transmitted Power $P$~[dBm]}, %Nombre eje X
    ylabel shift=-2ex,
     xlabel shift=-2ex,
    ylabel={Average BER~$\bar{P_\text{b}}$}, %Nombre eje X
    xtick={-5,-3,...,13},    %Similar al ajuste del grid del eje X, pero cuidado, porque es logarítmico 
    grid=major% axis on top
]

%----------LEYENDA-----------------
\addplot [color=black,solid,line width=1pt,mark options={solid}]coordinates {
         (10,1) (10,2)};\label{Orig_var1_jit12_black}
\addplot [color=black,dashed,line width=1pt,mark options={solid}]coordinates {
         (10,1) (10,2)};\label{Dashed_black}
\addplot [color=black,dotted,line width=1pt,mark options={solid}]coordinates {(10,1) (10,2)};\label{dotted_black}
 \addplot [only marks, color=black, mark=*, mark options={solid,scale=0.8, fill=white}]coordinates {(0.35,1)};\label{MC}
\addplot [name path=lim, color=FEC, very thick]
coordinates {(10,1) (10,2)}; \label{FEClimit}

  
%-------varR=1 Jiiter=0.12-------------

\addplot [ color=my_g,dashed,line width=1pt,mark options={solid}] file {./txtData/UpperBound/varR1_jit12/OOK_aprox1.txt};

\addplot [color=my_g,dotted,line width=1pt,mark options={solid}] file{./txtData/UpperBound/varR1_jit12/OOK_aprox2.txt};

%----MONTE CARLO----
\addplot [only marks, color=my_g, mark=*, mark options={solid,scale=0.8, fill=white}]file{./txtData/MC_3km/BER_MC_orig_varR1_jit12.txt};\label{MC_orig_var1_jit12}


%-----varR=0.1---jitter 0.35-----

\addplot [color=my_pink,solid,line width=1pt,mark options={solid}]file{./txtData/BER_3km/BER_orig_varR01_jit35.txt};\label{Orig_var01_jit35}

\addplot [ color=my_pink,dashed,line width=1pt,mark options={solid}] file{./txtData/UpperBound/varR01_jit35/OOK_aprox2.txt};
    
\addplot [color=my_pink,dotted,line width=1pt,mark options={solid}] file{./txtData/ICTON/Aprox2_varR01_jit35.txt};


%----MONTE CARLO----

\addplot [only marks, color=my_pink, mark=*, mark options={solid,fill=white,scale=0.8}]file{./txtData/MC_3km/BER_MC_orig_varR01_jit35.txt};\label{MC_orig_var01_jit35}


%------------FEC LIMIT
  \addplot [name path=lim, color=FEC, very thick]
   coordinates {(-15,3.84e-3) (14,3.84e-3)};


%------varR0.5------JITTER 0.25--------------

\addplot [color=orange,solid,line width=1pt,mark options={solid}] file {./txtData/BER_3km/BER_orig_varR05_jit25.txt};\label{Orig_var05_jit25}

\addplot [color=orange,dashed,line width=1pt,mark options={solid}] file{./txtData/UpperBound/varR05_jit25/OOK_aprox2.txt};
    
\addplot [color=orange,dotted,line width=1pt,mark options={solid}] file{./txtData/ICTON/Aprox2_varR05_jit25.txt};


%----MONTE CARLO----
\addplot [only marks, color=orange, mark=*, mark options={solid,scale=0.8,fill=white}]file{./txtData/MC_3km/BER_MC_orig_varR05_jit25.txt};\label{MC_orig_var05_jit25}

 
\end{semilogyaxis} %Finalizamos el diseño de la gráfica en sí


\node [draw,fill=white,anchor= south west,font=\scriptsize] at (0.05,0.05) {\shortstack[l]{ 
%\ref{Mix:W3_d50}  \hspace{0.025cm} \mbox{Curva 3}\\ 
\ref{Orig_var1_jit12_black} \hspace{0.01cm} \cite[Eq.~(16)]{ICTON} \\
\ref{Dashed_black} \hspace{0.01cm}  Eq. \eqref{eq:BER_UpperBound}\\
%\ref{Aprox2} \hspace{0.01cm} Eq. \mbox{HOLA}\\
 \ref{dotted_black} \hspace{0.01cm}  Eq. \eqref{eq:BER_Approx2_UpperBound}\\
 \hspace{0.15cm}   \ref{MC} \hspace{0.24cm}  Monte-Carlo\\
%\hspace{0.15cm}   \ref{MC_aprox1_var1_jit12} \hspace{0.24cm}  Monte Carlo $f_H(h)'$\\
  \ref{FEClimit} \hspace{0.01cm}  HD-FEC limit}};



\node [coordinate](input) {};


\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(2.22,9.3em)$) -- ($(input.north)+(2.22,7.3em)$);
\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(2.27,9.3em)$) -- ($(input.north)+(2.27,7.3em)$);
\node at ($(input.north) + (1.85, 6.8 em)$) [color=red, scale=1, font=\scriptsize] {$\Delta\approx0.17$~dB};

\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(4.6,9.3em)$) -- ($(input.north)+(4.6,8em)$);
\node at ($(input.north) + (4.6, 7.6em)$) [color=red, scale=1, font=\scriptsize] {$\Delta\approx0$~dB};

\draw[-,dashed, black,line width=0.5pt] ($(input.north)+(3.35,9.3em)$) -- ($(input.north)+(3.35,7.2em)$);
\node at ($(input.north) + (3.5, 6.7 em)$) [color=red, scale=1, font=\scriptsize] {$\Delta\approx0.006$ dB};


%DELTA2
% \draw[-,dashed, black,line width=0.5pt] ($(input.north)+(2.22,9.4em)$) -- ($(input.north)+(2.22,10.7em)$);
% \draw[-,dashed, black,line width=0.5pt] ($(input.north)+(2.29,9.4em)$) -- ($(input.north)+(2.29,10.7em)$);
% \node at ($(input.north) + (2.28, 11 em)$) [color=red, scale=1, font=\scriptsize] {$\Delta_2\approx0.21$ dB};

% \draw[-,dashed, black,line width=0.5pt] ($(input.north)+(4.6,9.3em)$) -- ($(input.north)+(4.6,11.9em)$);
% \node at ($(input.north) + (4.8, 12.4 em)$) [color=red, scale=1, font=\scriptsize] {$\Delta_2\approx0.1$ dB};

% \draw[-,dashed, black,line width=0.5pt] ($(input.north)+(3.35,9.3em)$) -- ($(input.north)+(3.35,11.7em)$);
% \node at ($(input.north) + (3.4, 11.8 em)$) [color=red, scale=1, font=\scriptsize] {$\Delta_2\approx0.08$ dB};

%Ellipse
\node[ellipse, draw,minimum width = 0.6cm, 
	minimum height = 0.05cm, rotate=45] (e) at (1.1,5.3) {};
\node at ($(input.north) + (0.7, 13.8em)$) [scale=1, font=\scriptsize] {$\sigma_s=0.35$ m};
\node at ($(input.north) + (0.7, 13.1em)$) [scale=1, font=\scriptsize] {$\sigma_R^2=0.1$};
 
\node[ellipse, draw,minimum width = 0.6cm, 
	minimum height = 0.05cm,rotate=45] (e) at (2.9,5) {};
\node at ($(input.north) + (3.6, 16em)$) [scale=1, font=\scriptsize] {$\sigma_s=0.12$ m};
\node at ($(input.north) + (3.5, 15.3em)$) [scale=1, font=\scriptsize] {$\sigma_R^2=1$};

\node[ellipse, draw,minimum width = 0.6cm, 
	minimum height = 0.05cm,rotate=45] (e) at (4.55,1.2) {};
\node at ($(input.north) + (3.9, 2.4em)$) [scale=1, font=\scriptsize] {$\sigma_s=0.25$ m};
\node at ($(input.north) + (3.9, 1.7em)$) [scale=1, font=\scriptsize] {$\sigma_R^2=0.5$};
 
\end{tikzpicture}

==> Sections/System_fig.tex <==
\definecolor{ashgrey}{rgb}{0.75, 0.75, 0.75}
\definecolor{antiquebrass}{rgb}{0.98, 0.81, 0.69}
\definecolor{brilliantlavender}{rgb}{0.96, 0.73, 1.0}

\tikzstyle{block} = [draw, line width = 1pt, fill=black!20, rectangle, minimum height=30pt, rounded corners=0.1cm, text width=2.2em,align=center]
    
\tikzstyle{block2} = [draw, line width = 1pt, fill=black!20, rectangle, minimum height=30pt, minimum width=30pt, rounded corners=0.1cm, text width=5em,align=center]


\tikzstyle{Cir} = [draw, circle,  minimum size=2.15em]

\begin{tikzpicture}[auto, node distance=1 cm,>=to,line width=0.5pt]

    %%%% IM/DD
    %% placing the blocks
    % TX 
    \node [coordinate] (input) {};
    \node [block, right = 2.2em of input, fill = antiquebrass] (OOK) {OOK}; 
    \node [block,right = 2.2em of OOK, fill = green!20] (INTER) {$\Pi$};
    \node [block,right = of INTER, fill = brilliantlavender] (EO) {E/O};
    
    % RX
    \node [block, right = 5 cm of EO, fill = brilliantlavender] (OE) {O/E}; 
    \node [block, right = of  OE, fill = green!20 ] (INTER2) {$\Pi^{-1}$};
    \node [block, right = 2.2em of  INTER2, fill = antiquebrass ] (HD) {HD};
    \node [right = 2.5em of  HD] (output) {};

        
    %Channel
   % \node [block2, align=center,text width=5em,at = ($(OOK.east)!0.5!(DeMOD.west)$), fill = green!20] (Chn)  {Fiber Channel}; 

    
    % We draw edges between nodes
    \draw [draw,->] (input) -- node[midway,above]{$b_k$} (OOK);
    \draw [draw,->] (OOK) -- node[midway,above]{$x_k$} (INTER); 
    \draw [draw,->] (INTER) -- node[midway,above]{$\tilde{x}_k$}(EO); 
    
    %\draw [draw,->] (INTER) -- node[midway,above]{symbol} node[midway,below](xi){$x_i$} (EO);  

   % \draw [draw,blue,line width=1pt,->] (Chn) -- node[midway,above,black,text width=5em, align = center]{optical waveform} (DeMOD);
    \draw [draw,->] (OE) -- node[midway,above]{$\tilde{y}_k$}(INTER2);
    \draw [draw,->] (INTER2) -- node[midway,above]{$y_k$} (HD);
    \draw [draw,->] (HD) --  node[midway,above,yshift=0.2em,text width=5em, align = center]{ $\hat{b}_k$}(output);

    %% Reference lines

%%DISTANCE LINE

    \draw [draw,black,line width=0.1pt,<->] ($(EO.east)+(0.3,-1.45)$) -- node[midway,above=8.5em,black,text width=5.5em, align = center]{Eq. \eqref{ChannelEq}} node[midway,above=0em,black,text width=5.5em, align = center]{$L$} ($(OE.west)+(-0.55,-1.45)$);
    
    
    \draw[dashed,very thick] ($(EO.south)+(-0.7,6em)$) -- ($(EO.south)+(-0.7,-3em)$);
    \draw[dashed,very thick] ($(EO.south)+(-0.7,6em)$) -- ($(OE.south)+(0.7,6em)$);
    \draw[dashed,very thick] ($(OE.south)+(0.7,6em)$) -- ($(OE.south)+(0.7,-3em)$);
    \draw[dashed,very thick] ($(EO.south)+(-0.7,-3em)$) -- ($(OE.south)+(0.7,-3em)$);

% CHANNEL 
    \draw[solid,line width=0.5pt] ($(EO.east)+(0.3,0.2em)$) -- ($(OE.west)+(-0.55,3.8em)$);
     \draw[solid,line width=0.5pt] ($(EO.east)+(0.3,-0.2em)$) -- ($(OE.west)+(-0.55,-3.8em)$);
     
     %Line between tx and rx$
      \draw[dashed,line width=0.5pt] ($(EO.east)+(0.25,0em)$) -- ($(OE.west)+(-0.5,0em)$);
  
\draw [solid,line width=1pt,rotate=90,fill=ashgrey,opacity=1] ($(EO.east)+(0,-0.3)$) ellipse (2.5mm and 1mm) node[at=($(EO.east)$),yshift=-2.5em, xshift=0.5cm,scale=1]{FSO Tx};

\draw [solid,line width=1pt,rotate=90,fill=ashgrey, opacity=1] ($(OE.west)+(0,0.55)$) ellipse (7mm and 3mm)node[at=($(OE.west)$),yshift=-2.5em, xshift=-0.8cm,scale=1]{FSO Rx};

\draw[latex-latex]  ($(EO.east)+(2.7,2.3em)$) arc(35:-6:1.2) node[midway,right]{$\theta_{1/2}$};

  %  \draw[solid,line width=0.5pt, <->] ($(OE.south)+(-2,3.8em)$) -- ($(OE.south)+(-2,-0.8em)$)  node[midway,left]{$2a$};;
    
 \draw[solid,line width=0.5pt, latex-latex] ($(OE.south)+(-1.05,3.55em)$) -- ($(OE.south)+(-1.05,1.45em)$)node[at=($(OE.west)$),yshift=1em, xshift=-0.67cm,scale=1]{$a$};;

 \draw[solid,line width=0.5pt, latex-latex] ($(OE.south)+(-0.65,5.35em)$) -- ($(OE.south)+(-0.66,-2.4em)$)node[at=($(OE.west)$),yshift=2.5em, xshift=0.1cm,scale=1]{$w_z$};;

%Phenomena
\draw[draw, -latex]  ($(EO.east)+(1.8,2.1em)$) arc(25:-1:1.2) node[at=($(EO.east)$),xshift=5em, yshift=2.8em,scale=1]{$h_p$};
\draw[draw, -latex]  ($(EO.east)+(1.3,2.1em)$) arc(25:-2:1.2) node[at=($(EO.east)$),xshift=3.5em, yshift=2.8em,scale=1]{$h_a$};
\draw[draw, -latex]  ($(EO.east)+(2.3,2.2em)$) arc(25:-1:1.2) node[at=($(EO.east)$),xshift=6.5em, yshift=2.8em,scale=1]{$h_l$};


%Lineas connect E/O to tx y rx
\draw [draw,-] (EO) --  ($(EO.east)+(0.2,0)$); 
\draw [draw,-] (OE) --  ($(OE.west)+(-0.27,0)$); 
\draw[solid,line width=0.7pt, <-] ($(OOK.north)+(0,0)$) -- ($(OOK.north)+(0,1.4em)$);
\node[at=($(OOK.north)$),yshift=1.9em,scale=1] { $2P$};



     
\end{tikzpicture}
